ICASSP 2022 Deep Noise Suppression Challenge

The Deep Noise Suppression (DNS) challenge is designed to foster innovation in the area of noise suppression to achieve superior perceptual speech quality. This is the 4th DNS challenge, with the previous editions held at INTERSPEECH 2020, ICASSP 2021, and INTERSPEECH 2021. We open-source datasets and test sets for researchers to train their deep noise suppression models, as well as a subjective evaluation framework based on ITU-T P.835 to rate and rank-order the challenge entries. We provide access to DNSMOS P.835 and word accuracy (WAcc) APIs to challenge participants to help with iterative model improvements. In this challenge, we introduced the following changes: (i) Included mobile device scenarios in the blind test set; (ii) Included a personalized noise suppression track with baseline; (iii) Added WAcc as an objective metric; (iv) Included DNSMOS P.835; (v) Made the training datasets and test sets fullband (48 kHz). We use an average of WAcc and subjective scores P.835 SIG, BAK, and OVRL to get the final score for ranking the DNS models. We believe that as a research community, we still have a long way to go in achieving excellent speech quality in challenging noisy real-world scenarios.

==> junk.tex <==
%The Blind test set is planned to include testclips recorded on desktop as well as mobile in realistic noisy environments.  
% \subsection{What's New}
%and another Azure service for DNSMOS P.835~\cite{reddy2021dnsmos} which is a deep neural network (DNN) model for prediction of speech, background noise, and overall quality.
%
% We also provide P.835 subjective evaluation framework and its modified version for PDNS evaluation. 
% Subjective test ITU-T P.835~\cite{naderi2020_p835} provides three scores for each audio clip, namely speech quality (SIG), background noise quality (BAK), and overall quality (OVRL). 
% Previous editions of the DNS Challenge provided researchers with a massive training dataset and real test set along with a P.808/P.835 test framework for subjective evaluation of enhanced speech. 
% Models which do well in all four metrics namely SIG, BAK, OVRL, and WAcc are ranked higher. 
%by cleaning the clean speech further and added some more data to capture relevant DNS scenarios. We collected a new test set for fullband speech ensuring high energy content in higher frequency bands to eliminate bandlimited clips from some devices. We included some new noise types in the test set covering contemporary scenarios and device variety. Our training data synthesizer script is flexible to allow the exclusion of any subset or addition of new data by the challenge participants. This provides an opportunity for leveraging challenge data along with other corpora for improving DNS performance. Our test set consists of real-world test clips recorded by crowd-sourced workers and Microsoft employees. We have two dev-test sets for real-time denoising and personalized real-time denoising. Similarly, we collect two blind tests set one for each challenge track. 
--
%However, the training and the test datasets did not include clean speech with emotions such as crying, yelling, laughter or singing. Also, the dataset only includes the English language. For DNS Challenge 2, we are adding speech clips with other emotions and included about 10 non-English languages. Clean speech in training set is total 760.53 hours: read speech (562.72 hours), singing voice (8.80 hours), emotion data (3.6hours), Chinese mandarin data (185.41 hours). We have grown clean speech to 760.53 hours as compared to 562.72 hours in DNS Challenge 1.
%
% of releasing the clean speech and noise datasets is to provide researchers with an extensive and representative dataset to train their SE models. We initially released MSSNSD \cite{reddy2019scalable} with a focus on extensibility, but the dataset lacked the diversity in speakers and noise types. We published a significantly larger and more diverse data set with configurable scripts for DNS Challenge 1 \cite{reddy2020interspeech}. Many researchers found this dataset useful to train their noise suppression models and achieved good results. 
%Non-personalized training set consist of original audio from various corpora.
%
--
%
%sets for both tracks has approximately 1500 real testclips, while the personalized track has 2.5 minutes of enrollment speech for each primary talker included in personalized DNS test set. All testclips in development set was collected through crowdsourcing where workers recorded the audio in different acoustic scenarios using a variety of Desktop/Laptops. The blind test set for both tracks have 3000 testclips where 1500 testclips were recorded on mobile devices (Android); and rest 1500 testclips were recorded on Desktop/Laptop platforms. 
%
% test set with 1500 testclips on each platform.  we increased the test set by 100\% by adding emotion data, singing voice, non-English languages in Track 1 and real and synthetic clips for personalized DNS in Track 2. We used the  open sourced subjective evaluation framework based on ITU-T P.808 \cite{naderi2020open} for final evaluation of the challenge. We finally present the challenge results and encourage other researchers to use the datasets and the tools to make significant progress.
% , and P.835 and P.808 subjective test frameworks. In the current challenge, we improved the training dataset by cleaning the previous corpora and added more clean speech for training. We added newer categories of real test clips in the test set such as mouse clicks and scroll wheels. 
%, 
%
%subjective evaluation to benchmark SE methods using a realistic noisy test set \cite{reddy2020interspeech}. We open sourced clean speech and noise corpus with configurable scripts to generate noisy-clean speech pairs suitable to train a supervised noise suppression model. There were two tracks, real-time and non-real-time based on the computational complexity of the inference. We received an overwhelming response to the challenge with participation from a diverse group of researchers, developers, students, and hobbyists from both academia and industry. We also received positive responses from the participants as many found the open sourced datasets quite useful, and both the dataset and test framework have been cloned at a fast rate since the chal
%
% The Deep Noise Suppression (DNS) Challenge organized at INTERSPEECH 2020 showed promising results, while also indicating that we are still about 1.4 Differential Mean Opinion Score (DMOS) from the ideal Mean Opinion Score (MOS) of 5 when tested on the DNS Challenge test set~\cite{valin2020perceptually, isik2020poconet}. 
% The DNS Challenge is the first contest that we are aware of that used subjective evaluation to benchmark SE methods using a realistic noisy test set \cite{reddy2020interspeech}. We open sourced clean speech and noise corpus with configurable scripts to generate noisy-clean speech pairs suitable to train a supervised noise suppression model. There were two tracks, real-time and non-real-time based on the computational complexity of the inference. We received an overwhelming response to the challenge with participation from a diverse group of researchers, developers, students, and hobbyists from both academia and industry. We also received positive responses from the participants as many found the open sourced datasets quite useful, and both the dataset and test framework have been cloned at a fast rate since the challenge.    
%
% clean speech which included singing voice, emotion data, and non-english languages (Chinese). Noise data in training set was same as the DNS Challenge 1. We provided over 118,000 room impulse responses (RIR), which includes real and synthetic RIRs from public datasets. 
% We also provided acoustic parameters: Reverberation time (T60) and Clarity (C50) for each read clean speech and RIR sample. 
% Noise suppression has become more important than ever before due to the increasing use of voice interfaces for various applications. Given millions of internet-connected devices being employed for audio/video calls, noise suppression is expected to be effective for all noise types chosen from daily-life scenarios.
%
% Participants will get access to a 4-page challenge paper, training dataset, baseline models, and dev-test set as soon as the grand challenge starts. The blind test set will be released shortly before the paper submission deadline to provide a test set on which final models will be evaluated. The blind test set ensures the generalizability of the DNS models submitted for this challenge. Challenge winners will be decided based on all the metrics SIG, BAK, OVRL, SRAR computed on enhanced data from the blind test set.  
%
% However, not many participants used the tool during their development phase as the subjective evaluation takes time and costs money. Most of the commonly used objective metrics like PESQ, POLQA, and SDR require a reference clean speech to compute the scores. Hence, we cannot use them on real recordings. Also, these metrics are shown to correlate poorly with subjective scores. We are providing a non-intrusive objective metric called Deep Noise Suppression MOS (DNSMOS) as an Azure service. DNSMOS is shown to correlate very well with subjective ratings and helps to stack rank the developed noise suppressors. 
%The final evaluation of the participating models were done based on subjective evaluation using the P.808 subjective testing framework. We describe the results of the challenge at the end.
% It is important to note that DNSMOS might not be applicable for stacking ranking Track
% With decades of research, deep noise suppression (DNS) has advanced to improve subjective overall audio quality while we are still quite far from eliminating speech distortions that result from over-suppression of noise. Preserving speech quality (i.e., eliminating speech distortion) and suppressing noise are two trade-offs DNS models must handle.
--
%with Creative Commons Attribution 4.0 International License (CC BY 4.0).
% to sort the book chapters by subjective quality. The audio chapters in Librivox are of variable length ranging from few seconds to several minutes. We randomly sampled 10 audio segments from each book chapter, each of 10 seconds in duration. For each clip, we had 2 ratings, and the MOS across all clips was used as the book chapter MOS. Figure 1 shows the results, which show the quality spanned from very poor to excellent quality. In total, it is 562 hours of clean speech, which was part of DNS Challenge 1.
% We downsampled the mono .WAV files from 44.1kHz to 16kHz and added it to clean speech used by the training data synthesizer. 
%
%The third subset consists of emotion speech recorded in noise-free conditions. This is derived from Crowd-sourced Emotional Mutimodal Actors Dataset (CREMA-D)~\cite{cao2014crema} made available under the Open Database License. It consists of 7,442 audio clips from 91 actors: 48 male, and 43 female accounting to total 3.5 hours of audio. The age of the actors was in the range of 20 to 74 years with diverse ethnic backgrounds including African America, Asian, Caucasian, Hispanic, and Unspecified. Actors read from a pool of 12 sentences for generating this emotional speech dataset. It accounts for six emotions: Anger, Disgust, Fear, Happy, Neutral, and Sad at four intensity levels: Low, Medium, High, Unspecified. The recorded audio clips were annotated by multiple human raters in three modalities: audio, visual, and audio-visual. Categorical emotion labels and real-value emotion level values of perceived emotion were collected using crowd-sourcing from 2,443 raters. This data was provided as 16 kHz .WAV files so we added it to our clean speech as it is. 
%
% Non-English languages has Ch It consists of both tonal and non-tonal languages including Chinese (Mandarin), German and Spanish. Mandarin data consists of OpenSLR18~\footnote{http://www.openslr.org/18/} THCHS-30~\cite{THCHS30_2015} and OpenSLR33~\footnote{http://www.openslr.org/33/} AISHELL~\cite{aishell_2017} datasets, both with Apache 2.0 license. THCHS30 was published by Center for Speech and Language Technology (CSLT) at Tsinghua University for speech recognition. It consists of 30+ hours of clean speech recorded at 16-bit 16 kHz in noise-free conditions. Native speakers of standard Mandarin read text prompts chosen from a list of 1000 sentences. We added the entire THCHS-30 data in our clean speech for the training set. It consisted of 40 speakers: 9 male, 31 female in the age range of 19-55 years. It has total 13,389 clean speech audio files~\cite{THCHS30_2015}. The AISHELL dataset was created by Beijing Shell Shell Technology Co. Ltd. It has clean speech recorded by 400 native speakers ( 47\% male and 53\% female) of Mandarin with different accents. The audio was recorded in noise-free conditions using high fidelity microphones. It is provided as 16-bit 16kHz .wav files. It's one of the largest open-source Mandarin speech datasets. We added the entire AISHELL corpus with 141,600 utterances spanning 170+ hours of clean Mandarin speech to our training set.
%
%Non-personalized track contains original audio clips from different corpora and corresponding DNSMOS scores so participants can choose to use audio clips with DNSMOS P.835 OVRL score of 4. In total, Spanish clean speech is 46 hours,  of clean speech z. German data is derived from four corpora namely (i) The Spoken Wikipedia Corpora~\cite{swc}, (ii) Telecooperation German Corpus for Kinect~\cite{kinect}, (iii) M-AILABS data~\cite{mailabs}, (iv) zamia-speech forschergeist corpora. Complete German data constitute 636 hours. Italian (128 hours), French (190 hours), Russian (47 hours) are taken from M-AILABS data~\cite{mailabs}. M-AILABS Speech Dataset is a publicly available multi-lingual corpora for training speech recognition and speech synthesis systems.
%


--

% , both released with Apache 2.0 License.
%%
% \vspace{-1mm}
% \subsection{Acoustic parameters}
% We provide two acoustic parameters: (i) Reverberation time, T60~\cite{antsalo2001estimation} and (ii) Clarity, C50~\cite{gamper2020blind} for all audio clips in clean speech of training set. We provide T60, C50 and isReal Boolean flag for all RIRs where isReal is 1 for real RIRs and 0 for synthetic ones. The two parameters are correlated. A RIR with low C50 can be described as highly reverberant and vice versa~\cite{antsalo2001estimation,gamper2020blind}. These parameters are supposed to provide flexibility to researchers for choosing a sub-set of provided data for controlled studies. 
%
%\vspace{-2mm}
%
%\vspace{-1mm}
%\subsubsection{Real recordings}
%\label{sssec:realrec}
%
%
% \vspace{-1mm}
% \subsubsection{Synthetic test set}
% \label{sssec:synth}
% The synthetic test set consisted of 200  noisy clips obtained by mixing clean speech (non-English, emotional speech, and singing) with noise. The test set noises is taken from Audioset and Freesound~\cite{reddy2020interspeech}. The 100 non-English test clips include German, French and Italian languages from Librivox audio books.  Emotion clean speech consists of laughter, yelling, and crying chosen from Freesound and mixed with test set noise to generate 50 noisy clips. Similarly, clean singing voice from Freesound was used to generate 50 noisy clips for the singing test set. 
%in the presence of background noise and the remaining 50 clips include singing in the presence of background noise.   
%
% \subsubsection{Blind test set}
% \label{sssec:blind}
% The blind test set for track 1 contains 700 noisy speech clips out of which 650 are real recordings and 50 synthetic noisy singing clips. It contains the following categories: (i) emotional (102 clips), (ii) English (276 clips), (iii) non-English including tonal (272 clips), (iv) tonal languages (112 clips) and (v) singing (50 clips). The real recordings were collected using the crowdsourcing platform and internally at Microsoft. This is the most diverse publicly available test set for a noise suppression task.
%

--

%
%that can be used to adapt the model to better suppress any background noise other than that particular speaker's voice. In the datasets directory. The track 2 test clips can be found in the \textbf{track\_2} sub-directory of \textbf{ICASSP\_dev\_test\_set}.The 2 mins data per speaker that can be used for adaptation is provided in the \textbf{adaptation\_data} directory. The noisy speech for each of these speakers is in \textbf{noisy} directory.adaptation must happen during the inference.  
%
%\subsubsection{Blind test set}
%\label{sssec:blind}
%The blind test set for track 2 contains 500 noisy speech real recordings from 80 unique speakers. All the real recordings were collected using the crowdsourcing platform. The noise source in the majority of these clips is a secondary speaker. We provided 2 mins clean speech utterances for each of the primary speakers that could be used to adapt the noise suppressor. All the utterances were in English.

% \section{DNSMOS: A No-reference Objective speech quality metric}
% We developed a robust objective perceptual speech quality metric called DNSMOS. It can be used to stack rank different DNS methods based on Mean Opinion Score (MOS) estimates with great accuracy. It is a neural network-based model that is trained using the ground truth human ratings obtained using ITU-T P.808 \cite{naderi2020open, reddy2020interspeech}. The audio data used to train the DNSMOS model is gathered from the numerous P.808 experiments that we conducted in the process of improving the quality of noise suppressor. DNSMOS is trained on the largest and the most extensive data set that we are aware of. We were able to achieve a Spearman rank correlation coefficient of 0.96 with subjective human ratings on the DNS Challenge 1 blind test set using the 28 submitted models.
%
% Sample code and details of the evaluation API can be found on \url{https://dns-challenge.azurewebsites.net/dnsmos/ICASSP2021}
%
%
--
% RawNet2-modified 
% We opensource speaker embedding extractor so that participants could use it on newer corpora. For this purpose, we leverage a publicly available speaker embedding extractor RawNet2-modified~\cite{jung2020improved}.2480] ResNeXt and Res2Net Structures for Speaker Verification (arxiv.org). 
% The development test set contains 100 real recordings from 20 primary speakers collected using crowdsourcing. Each primary talker has noisy test clips for three scenarios: (i) primary talker in presence of neighboring  talker; (ii) primary talker in presence of background noise; and (iii) primary talker in presence of both background noise and neighboring  talker. The synthetic clips include 500 noisy clips from 100 primary speakers. Each primary talker has 2 minutes of clean adaptation data. All clips have varying levels of neighboring talkers and noise. test set noise from Track 1 was mixed with primary speech extracted from VCTK corpus~\cite{yamagishi2019cstr}. We used VoxCeleb2~\cite{chung2018voxceleb2} corpus for neighboring talkers.
%
% Since public speaker models were trained on 16kHz data, participants can start their experimentation by down-sampling the fullband enrollment data to 16 kHz for extracting speaker embeddings for their pDNS models. 
%
% Since speaker embeddings from fullband data (48kHz) are likely to provide better pDNS performance, participants need to re-train speaker embedding extractor on 48kHz data during their development stages.  To validate the feasibility of pDNS, our baseline personalized pDCCRN model needs to show better DSIG and DMOS for Track 2 test set than the non-personalized pDCCRN model.
%
%\begin{table}[t!]
%  \begin{center}
%\vspace{-3mm}
% \caption{Performance of baseline models on Dev test set.}
% \vspace{-3mm}
% \label{tab:baseline_results}
% \begin{tabular}{|l|r|r|r|r|}
%   \hline
%   \textbf{Model} & \hspace{-1mm}\textbf{test set} & \textbf{DSIG} & \textbf{DBAK} & \textbf{DOVRL} \\
%   \hline NSNet2 & Non-personalized dev test set  &   &  &  \\ 
%   \hline pDCCRN &  Personalized dev test set  &  & & \\
%   \hline Personalized CRUSE &  Track 2 test set &   &  &  \\
%   \hline
%\end{tabular}
% \end{center}
%\end{table}
%%
%\vspace{-2mm}
%\section{Challenge Results}
%\vspace{-1mm}

--

%The first 6 seconds of each appended clip are intended to make workers aware of the primary talker's speech. 
% We conducted a reproducibility test for modified P.835 and found the average Spearman Rank Correlation Coefficient (SRCC) between the 5 runs was {}. Hence, we can conclude that the modified P.835 is working as intended. For reproducibility study, we used 5 raters per clip, resulting in a 95\% confidence interval (CI) of 0.03. 

